diffpy.morph: Python tools for model independent comparisons between sets of 1D functions

diffpy$.$morph addresses a need to gain scientific insights from 1D scientific spectra in model independent ways. A powerful approach for this is to take differences between pairs of spectra and look for meaningful changes that might indicate underlying chemical, structural, or other modifications. The challenge is that the difference curve may contain uninteresting differences such as experimental inconsistencies and benign physical changes such as the effects of thermal expansion. diffpy$.$morph allows researchers to apply simple transformations, or "morphs", to one of the datasets to remove the unwanted differences revealing, when they are present, non-trivial differences. diffpy$.$morph is an open-source Python package available on the Python Package Index and conda-forge. Here, we describe its functionality and apply it to solve a range of experimental challenges on diffraction and PDF data from x-rays and neutrons, though we note that it may be applied to any 1D function in principle.

==> cmds_general.tex <==
%% Diffraction specific things
\newcommand{\kalpha}{\ensuremath{K_\alpha}\xspace}
\newcommand{\kbeta}{\ensuremath{K_\beta}\xspace}

%% PDF-specific things
\newcommand{\qmax}{\ensuremath{Q_{\mathrm{max}}}\xspace}
\newcommand{\qmaxinst}{\ensuremath{Q_{\mathrm{max-inst}}}\xspace}
\newcommand{\qmin}{\ensuremath{Q_{\mathrm{min}}}\xspace}
\newcommand{\qbroad}{\ensuremath{Q_{\mathrm{broad}}}\xspace}
\newcommand{\qdamp}{\ensuremath{Q_{\mathrm{damp}}}\xspace}
\newcommand{\deltatwo}{\ensuremath{\delta_2}\xspace}
\newcommand{\deltaone}{\ensuremath{\delta_1}\xspace}
\newcommand{\spdiameter}{\ensuremath{sp_{\mathrm{diameter}}}\xspace}
\newcommand{\uiso}{\ensuremath{U_{\mathrm{iso}}}\xspace}
\newcommand{\uaniso}{\ensuremath{U_{\mathrm{aniso}}}\xspace}
\newcommand{\sratio}{\ensuremath{sratio}\xspace}
\newcommand{\rpoly}{\ensuremath{rpoly}\xspace}
\newcommand{\rw}{\ensuremath{R_w}\xspace}
\newcommand{\rapdf}{\textit{RA-PDF}\space}
\newcommand{\cif}{{\texttt{CIF}\xspace}
\newcommand{\rmin}{\ensuremath{r_{\mathrm{min}}}\xspace}
\newcommand{\rmax}{\ensuremath{r_{\mathrm{max}}}\xspace}
\newcommand{\rlim}{\ensuremath{r_{\mathrm{lim}}}\xspace}
\newcommand{\mmax}{\ensuremath{m_{\mathrm{max}}}\xspace}
\newcommand{\delr}{\ensuremath{dr}\xspace}
\newcommand{\delrn}{\ensuremath{dr_N}\xspace}
\newcommand{\delq}{\ensuremath{dQ}\xspace}
\newcommand{\qualp}{\ensuremath{\mathcal{Q}_p}\xspace}
\newcommand{\iq}{\ensuremath{I(Q)}\xspace}
\newcommand{\sq}{\ensuremath{S(Q)}\xspace}
\newcommand{\fq}{\ensuremath{F(Q)}\xspace}
\newcommand{\gr}{\ensuremath{G(r)}\xspace}
\newcommand{\rr}{\ensuremath{R(r)}\xspace}
\newcommand{\q}{\ensuremath{Q}\xspace}
\newcommand{\ir}{\ensuremath{r}\xspace}
\newcommand{\dd}{\ensuremath{\mathrm{d}}
\newcommand{\ii}{\mathrm{i}}
% we like our vectors to be bold and not italicised
\renewcommand{\vec}[1]{\mathbf{#1}}

%units
\newcommand{\iaa}{\AA\ensuremath{^{-1}}\xspace}
\newcommand{\iaasquared}{\AA\ensuremath{^{-2}}\xspace}
\newcommand{\aasquared}{\AA\ensuremath{^{2}}\xspace}

% comments
% Add your own here. Pick your own color.
\newcommand{\sjb}[1]{\textcolor{blue}{[sjb:#1]}}
\newcommand{\sjba}[1]{}
\newcommand{\mt}[1]{\textcolor{orange}{[mt:#1]}}
\newcommand{\mta}[1]{}


% referencing figures etc. correctly
%
% when you make the label, use
% \label{fig:<name>} for figures
% \label{eq:<name>} for equations and so on (see below for what to use}
%
% Never use numbers for anything as the numbering always changes.  The point
% is to use a <name> that is descriptive (and preferrably memorable)
%
% when you then reference the item reference it like
% "...as is evident in \fig{<name>}" and will compile as "...as evident in Fig. 4"
\newcommand{\eq}[1]{Eq.~\ref{eq:#1}}
\newcommand{\eqs}[1]{Eqs.~\ref{eq:#1}}
\newcommand{\fig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figs}[1]{Figs.~\ref{fig:#1}}
\newcommand{\sect}[1]{Section~\ref{sec:#1}}
\newcommand{\apen}[1]{Appendix~\ref{sec:#1}}
\newcommand{\tabl}[1]{Table~\ref{table:#1}}
\newcommand{\bra}[1]{\left<#1\right|}
\newcommand{\ket}[1]{\left|#1\right>}
%\newcommand{\abs}[1]{\left|#1\right|}

% correctly formated latin
\newcommand{\etal}{\emph{et al.}\xspace}
\newcommand{\adhoc}{\emph{ad hoc}\xspace}
\newcommand{\insitu}{\emph{in situ}\xspace}
\newcommand{\operando}{\emph{operando}\xspace}


% Colored symbols used during editing.
% Also, define new colors here if you like
\definecolor{dgreen}{HTML}{008000}
\newcommand{\done}{\textcolor{dgreen}{{\large{$\checkmark$}}}}
\newcommand{\doing}{\textcolor{blue}{{\large{$\blacklozenge$}}}}
\newcommand{\checkme}{\textcolor{orange}{{\large{$\blacktriangleleft$}}}}
\newcommand{\fixme}{\textcolor{red}{{\large{$\blacktriangleright$}}}}

% some style preferences for code listings
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=mystyle}

% used for building skels.  If you want to jump out of the list and jump back in later do it this way:
% \be               % begin the enumerated list
% ...
% \seti\ee          % paus the list, saving the counter
% ...
% \be\conti         % continue the list from where we left off
% ...
% \ee               % end the list, it is the end of hte paper
\newcounter{saveenumi}
\newcommand{\seti}{\setcounter{saveenumi}{\value{enumi}}}
\newcommand{\conti}{\setcounter{enumi}{\value{saveenumi}}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bes}{\begin{enumerate}[wide, labelwidth=!, labelindent=0pt, label=\textbf{\textcolor{blue}{\arabic*}.}]}
\newcommand{\ees}{\end{enumerate}}


==> cmds_programs.tex <==
% Group program names.  Generally the pdf is dropped, so PDFgui is \gui
\newcommand{\plotdata}{{\sc plotdata}\xspace}
\newcommand{\getx}{{\sc PDFgetX3}\xspace}
\newcommand{\gui}{{\sc PDFgui}\xspace}
\newcommand{\itc}{{\sc PDFitc}\xspace}
\newcommand{\guitwo}{{\sc PDFgui2}\xspace}
\newcommand{\xsuite}{{\sc xPDFsuite}\xspace}
\newcommand{\esuite}{{\sc ePDFsuite}\xspace}
\newcommand{\cmi}{{\sc Diffpy-CMI}\xspace}
\newcommand{\morph}{{\sc PDFmorph}\xspace}
\newcommand{\srmise}{{\sc SrMise}\xspace}
\newcommand{\srfit}{{\sc SrFit}\xspace}
\newcommand{\srxplanar}{{\sc SrXplanar}\xspace}
\newcommand{\xpdacq}{{\sc xpdAcq}\xspace}
\newcommand{\xpdan}{{\sc xpdAn}\xspace}
\newcommand{\xpdtools}{{\sc xpdtools}\xspace}
\newcommand{\shed}{{\sc SHED}\xspace}
\newcommand{\pyfai}{{\sc PyFai}\xspace}
\newcommand{\mpdf}{{\sc diffpy.mpdf}\xspace}
\newcommand{\strumining}{{\sc structureMining}\xspace}
\newcommand{\clustermining}{{\sc clusterMining}\xspace}
\newcommand{\nmfmapping}{{\sc nmfMapping}\xspace}
\newcommand{\motexml}{{\sc MotEx-ML}\xspace}

% general program names
\newcommand{\jupyter}{{\sc Jupyter}\xspace}
\newcommand{\pycharm}{{\sc PyCharm}\xspace}


==> packages.tex <==
% place all figures in a sub-folder called figures, located in the folder where
% the main latex file is
%
% then when you include the graphics, do not put any path there
% e.g., \includegraphics[width=0.8\textwidth]{<name>}
% for a figure called <name>.pdf (or <name>.png, or <name>.jpg...latex will do
% its best to choose the extension from known image file types).
%
% as preference use pdf format files.  These are vector graphics and so produce
% higher quality images at all scales.
\graphicspath{ {./figures/} }

%
%Packages
%
\usepackage{enumitem}
\usepackage{xspace}
\usepackage{fancyhdr}
\usepackage{afterpage}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{dcolumn}
\usepackage{comment}
\usepackage{listings}
\usepackage{makeidx}
\usepackage{longtable}
\usepackage{chemformula}
\usepackage[utf8]{inputenc}
\usepackage{comment}

%get the floats right
\usepackage[dvips]{epsfig}
\usepackage{epstopdf}
\usepackage{graphicx}% Include figure files

%math packages for more advanced math
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{amsfonts}
\usepackage{commath} %http://ctan.mackichan.com/macros/latex/contrib/commath/commath.pdf
\usepackage[a4paper, total={6in, 9in}]{geometry}

